Approximate Nearest Neighbor Negative Contrastive Learning for Dense Text Retrieval

Conducting text retrieval in a dense learned representation space has many intriguing advantages over sparse retrieval. Yet the effectiveness of dense retrieval (DR) often requires combination with sparse retrieval. In this paper, we identify that the main bottleneck is in the training mechanisms, where the negative instances used in training are not representative of the irrelevant documents in testing. This paper presents Approximate nearest neighbor Negative Contrastive Estimation (ANCE), a training mechanism that constructs negatives from an Approximate Nearest Neighbor (ANN) index of the corpus, which is parallelly updated with the learning process to select more realistic negative training instances. This fundamentally resolves the discrepancy between the data distribution used in the training and testing of DR. In our experiments, ANCE boosts the BERT-Siamese DR model to outperform all competitive dense and sparse retrieval baselines. It nearly matches the accuracy of sparse-retrieval-and-BERT-reranking using dot-product in the ANCE-learned representation space and provides almost 100x speed-up.

==> Arxiv/Intro.tex <==
\section{Introduction}

\cx{
Our main contribution:
\begin{enumerate}
    \item A new ANN NCE training framework that provides more effective and aligned training for dense retrieval, fixed the mismatch in negatives in learning and inference
    \item the first to outperform sparse retrieval in real IR document tasks with pure dense retrieval and outperforms all previous dense retrieval/representation based retrieval methods by large 
    \item thorough analyses illustrating the ANN-NCE learning process and its influence. 
    % \ja{Can we allude to SOTA results on representation based information retrieval of relevant results ? done, #2}
\end{enumerate}
}

% \cx{Outlines. Each bracket is }



% \cx{where we are in language AI: beyond human in later stage, rule-based 40 years old BM25 in first stage}
Many NLP-focused systems rely on text retrieval to find relevant information as input for later inference stages. For example,
search ranking~\cite{nogueira2019passage}, answer span extraction~\cite{chen2017reading}, multi-hop reasoning~\cite{yang2018hotpotqa, thorne2018fact}, grounded conversation response generation~\cite{zhou2018dataset} all assume extracting from the broad set of all items a set of filtered ``mostly relevant'' candidates on which a more computationally expensive ranking, extraction, classification, or generation step is run. All these ``later stage modules'' have enjoyed the revolutionary advantages from distributed, pretrained, and end-to-end deep learning models, and reached ``beyond human performances'' in many public benchmarks~\cite{rajpurkar2016squad, wang2018glue}. In contrast, the first stage retrieval part, which provides the basic information for the later components in these AI systems, is often still based on the sparse, bag-of-words, representations and exact matches within~\cite{chen2017reading, zhaotransxh2020, yang2018hotpotqa, nogueira2019passage}.
BM25~\cite{bm25}, unsupervised sparse retrieval using hand-crafted rules, is still a strong baseline and sometimes even the state-of-the-art, 40 years after its invention~\cite{zamani2018neural, karpukhin2020dense, luan2020sparsedense, lee2019latent}.



The limited capability of the sparse first retrieval enforces a potential upper bound of modern language AI systems.
The intrinsic challenge of sparse retrieval, i.e. vocabulary mismatch and language varieties~\cite{croft2010search}, brings in noisy and missed information in the first stage, which is challenging, sometimes impossible \ao{should this statement be stronger? there should be many queries where context isn't captured by keyword matching, resulting in BM25 to miss the document at L1 which cannot be recovered from in later stages}, \ja{I would add that in a multi-step search process, the first step fundamentally limits the second step, which is what Arnold is also alluding to \cx{Yes. Now it is doing the same purpose but I should spend more space on the challenge part.}}for the later deep neural models to recover~\cite{yang2018hotpotqa, craswell2020overview}. 




% \cx{The importance of dense retrieval:
% \begin{enumerate}
%     \item resolve the bottleneck in e2e information system
%     \item unleash the full potential of neural methods in many downstream applications
%     \item unified and easier to maintain infrastructure
%     \item Also Pretrained LM and ANN inference are getting ready
% \end{enumerate}
% }
% \cx{The observations and challenges in recent progress:
% \begin{enumerate}
%     \item good for short passage but not as good on longer passage
%     \item reranking is promising but not yet fully e2e retrieval, many times have to combine with sparse model
%     \item even some permissive analyses that the capacity of encoding has to be very high for documents
% \end{enumerate}
% }

Dense retrieval, which learns retrieval texts using the learned distributed embeddings, is a promising potential direction to overcome the sparse retrieval bottleneck~\cite{lee2019latent, chang2020pre, luan2020sparsedense, gao2020complementing, ma2020zero, dhingra2020differentiable, karpukhin2020dense}: The representation space is end-to-end learned,  tailored for the task, leverages the strength of language model pretraining, while also being sufficiently efficient thanks to the recent progress in Approximate Nearest Neighbor (ANN) search~\cite{johnson2019billion}. \ja{minor point: I wonder if the statement above where we say that BM25 is state of the art and that dense retrieval already has many citations (and hence are proven better than BM25) could conflict ? \cx{citations is not equal to better, many dense retrieval paper show they are not as strong on longer texts.}}

One would expect learned dense representation to revolutionize the first stage retrieval, as they have in many other language tasks. However, this is not necessarily the case in text retrieval: Recent studies often found that dense retrieval with BERT sometimes under performs or is merely on-par with BM25, especially on long texts~\cite{luan2020sparsedense, lee2019latent}, raising concerns whether it is sustainable \ja{maybe a better way than sustainable is a more performant solution or has better ROI than BM25. \cx{Yes, it is a little subtle, we don't want to attack the ROI of our dense retrieval but need to say it was hard before this work.}} for document retrieval~\cite{luan2020sparsedense}, and the effectiveness of dense retrieval is mainly when combined with spare retrieval~\cite{gao2020complementing, ma2020zero}---as an add-on to BM25, but not yet a next-gen retrieval.





% \cx{Our solution:
% \begin{enumerate}
%     \item We identified the main bottleneck is actually in the training phrase, the mismatch between negatives seem in training and ANN inference
%     \item Developed a new training mechanism in the NCE framework, but instead of in-batch sampling, we directly do that in ANN, which is exact how the dense retrieval model is to be used
% \end{enumerate}
% }

In this paper we identify the main reason of such underwhelming performance of dense retrieval, especially on longer texts, is the learning part. Specifically, the mismatches of negatives sampled for training and the actually negatives in retrieval. 
% \ja{Previous sentence and next sentence are both technically strong and convey vital aspect of understanding; consider : Too many commas, suggest breaking down the long sentence for better readability}
In training, the negatives is either randomly sampled, selected in nearby batches, or from the sparse retrieval, following standard learning to rank settings~\cite{liu2009learning}. However, when testing, the trained model needs to retrieve the relevant documents in the entire corpus, e.g., via ANN, which is drastically different  from the negatives in sparse retrieval nor the random sampled negatives can provide the minutiae required for ranking among the top retrievals ($\mathsection$~\ref{sec:ancenegatives}). 


% \cx{More details of ANCE:
% \begin{enumerate}
%     \item We build ANN index with the doc representations
%     \item directly pick negatives from the ANN for each q and d+ label
%     \item refresh ANN after certain steps, as asynchronous updates
%     \item until converges in validation
% \end{enumerate}
% }

We eliminate this mismatch with Approximate nearest neighbor Noise Contrastive Estimation (ANCE), which follows the principle of NCE~\cite{gutmann2010noise, mnih2013learning, oord2018representation}, and selects stronger, \textit{more realistic}, negatives from an ANN index in learning. The ANN index includes the encodings of the documents/passages, from the same representation model being learned for the dense retrieval, and is parallelly updated and asynchronously refreshed as the optimization goes on. The negatives are sampled from this ANN index using the same retrieval function (dot product, e.g.), the same representation model (though delayed due to the asynchronous index update). Thus the training negatives are much more aligned with the actual negatives dense retrieval models would encounter in real world. \ja{Could we say that this is an "effective hard negative sampling problem" addressed through elegant use of lower ranked documents ? I personally found the analogy with hard negative which is a well known ML concept quite apt but not sure if that resonates with research community \cx{It is doing this? I will make the point more crisp. Note that NCE, InfoNCE is doing strong negative selection, we are just doing it better and more fundemental.}}





% \cx{Our contribution as shown in experiments:
% \begin{enumerate}
%     \item The first to outperform all sparse retrieval, BM25 and beyond, as well as feature-based LeToR on TREC DL Doc task, a realistic, large scale, document retrieval task from Bing queries and documents.  
%     \item stronger than other training mechanisms: NCE, in batch, BM25+NCE, etc. (hopefully also momentum).
%     \item All with vanilla BERT-Siamese,  works for both doc ranking and passage ranking, with simple max-pooling or longformer on doc side.
% \end{enumerate}
% }

In TREC Deep Learning Track's large scale document and passage ranking benchmarks~\cite{craswell2020overview}, ANCE significantly boost the retrieval accuracy of dense retrieval. With ANCE training, the vanilla BERT-Siamese dual encoder, the same architecture used in several parallel research~\cite{luan2020sparsedense, gao2020complementing, ma2020zero}, significantly outperforms all dense retrieval baselines, many with same architecture but different training scheme, and sparse retrieval methods, not only BM25, but also its stronger variations developed in core ad hoc retrieval.  
ANCE in fact empowers vanilla BERT-Siamese to outperform many two-stage retrieval-and-reranking systems~\cite{liu2009learning, www2017duet}, solely via one dense retrieval step with dot-product in the representation space. This overwhelming effectiveness
% \ja{overwhelming effectiveness} 
is the first we have seen in dense document retrieval, and our analyses provide further insights and illustrate how ANCE effectively trains the encoders for more robust and accurate dense retrieval.



% \cx{Our insights:
% \begin{enumerate}
%     \item the main gain is from our ANCE training, without it, there is a clear gap in reranking and retrieval, and our analyses show how the gap of different negatives are resolved during the ANCE training.
%     \item More details in how/when to refresh index, the LR scheduling, warm up, and negative sampling, to shine lights of representation learning in other related tasks
%     \item case studies to show the different behavior of dense retrieval and sparse retrieval 
% \end{enumerate}
% }

==> Arxiv/doc_res.tex <==
\lx{this is placeholder template until numbers are fully replaced}
\begin{table*}[ht]
    \centering
    \small
    % \begin{adjustbox}{width=0.95\textwidth,center}
    \begin{tabular}{l|cc|cc|cc} \hline \hline
    & \multicolumn{2}{c|}{\textbf{MARCO Dev}} 
    & \multicolumn{2}{c|}{\textbf{TREC Rerank}} 
    & \multicolumn{2}{c}{\textbf{TREC Retrieval}}
    \\ \hline  
    % \textbf{Method}     
    % &  \multicolumn{2}{c}{\textbf{Precision@1}} &  \multicolumn{2}{c}{\textbf{Precision@3}}  &  \multicolumn{2}{c|}{\textbf{Recall@5}}
    %   &  \multicolumn{2}{c}{\textbf{Precision@1}} &  \multicolumn{2}{c}{\textbf{Precision@3}}  &  \multicolumn{2}{c}{\textbf{Recall@5}}
    % \\ \hline
           \textbf{Method}     
    &  \textbf{MRR@10} &  \textbf{Recall@1k}
     &  \textbf{NDCG@10} &  \textbf{Hole@10}
     &  \textbf{NDCG@10} &  \textbf{Hole@10}
    \\ \hline
{BM25} 
& 0.31 & ~ & N/A & N/A & 0.52 & 2\% \\
{Best DeepCT}~\cite{dai2019context} & \\
{TREC Best Retrieval}  & \\
{TREC Best Trad} & 
\\ \hline
{BERT Ranker}~\cite{nogueira2019passage}  % from literature 
& -- & -- & 0.64 & ~  & -- & -- 
\\\hline

%
%{\textbf{*Document Warmup}} \cx{move this to appendix \lx{ablation study or appendix?} } & ~ & 0.35 & ~ & ~ & ~ & ~ & ~  \\ %/webdata-nfs/yeli1/msmarco_doc_5M_30k/rdot_nll_128_bm25/checkpoint-84000/
%{w/ ANCE - 512} & ~ & 0.56 & ~ & ~ & ~ & ~ & ~   \\
%\hline

{\textbf{Dense Retrieval}}   \\
BM25 $\rightarrow$ Random Neg \\
%checkpoint_path = "/mnt/azureblob/lexion/doc_checkpoint/"
%checkpoint = 0

{NCE Neg}~\cite{gutmann2010noise} \\

{BM25 + Random}~\cite{luan2020sparsedense, karpukhin2020dense} 
& ~ & ~ & 0.630 & 2.5\% & 0.539 & 26\%   \\
% checkpoint_path = "/webdata-nfs/lexion/msmarco_doc_5M_30k/final_IB_BM25_measure/"
%checkpoint = 0

{w. ANCE (512)} & ~ & ~ & 0.641 & 3\% & 0.615 & 13\%    \\ 
%checkpoint_path = "/mnt/azureblob/lexion/doc_checkpoint/"
%checkpoint = 210000

{w. ANCE (2048)} & ~ & ~ & ~ & ~ & 0.625 & ~ %checkpoint_path = "/webdata-nfs/yeli1/msmarco_doc_5M_30k/rdot_null_2048_lr1e-5/"
%checkpoint = 139000

\\

\hline \hline
    \end{tabular}
     \caption{TREC DL Track 2019 Document 
    \label{tab:doc_overal}}
%   \end{adjustbox}
\end{table*}



==> Arxiv/efficiency.tex <==
\begin{sbsfigure*}
\centering
\small
\begin{tabular}{l|c|c} \hline \hline
\textbf{Operation} & \textbf{Offline}  & \textbf{Online } \\ \hline
    {\textbf{Sparse \& Cascade IR }} & \\
    {BM25 Retrieval} & & TODO  \\
    {Bert Rerank} & & 1.15s  \\
    {BM25 $\rightarrow$ Bert Reranker}  & & BM25+1.15s \\ \hline
    
    {\textbf{Dense IR }} & \\
    {ANCE Doc Encoding} & 10h per 8m doc &  \\
    {ANCE Query Encoding} & & 2.6ms \\
    \hline
    {\textbf{ANN Lookup}} &   \\
    {10 Query Batch} & 0.3s \\
    {100 Query Batch} &  92ms \\
    {1k Query Batch} & 9ms
    \\\hline
    {\textbf{End-to-End}}  & \\
   
    {ANCE Embedding} & 11.6ms \\
    \hline\hline
    {\textbf{ANCE Training}} &  \\
    {ANCE Corpus Inference} & 10h \\
    {ANN Index Build} & 10s \\
    {ANCE Training Set Build } & 5m  \\
    {Encoder Backprop} & 19ms \\
    \hline
    \end{tabular}
\end{sbsfigure*}



==> Arxiv/efficiency_training_tbl.tex <==
\lx{TODO: place holder for runtime efficiencies}

\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{l|c} \hline \hline
      & \multicolumn{1}{c}{\textbf{Time}} 
    \\  \hline

{\textbf{ANCE Training}} &  \\
{ANCE Corpus Inference} & 10h \\
{ANN Index Build} & 10s \\
{ANCE Training Set Build } & 5m  \\
{Encoder Backprop (1query, 1 positive, 1 negative)} & 19ms
\\\hline


\hline \hline
    \end{tabular}
     \caption{Measurement performed on single 32GB V100 GPU, XXX CPU, 660GB Memory 
     ~\label{tab:train_efficiency}}
\end{table*}



==> Arxiv/eval.tex <==
\section{Evaluation Results}
\input{Tables/doc_pass_combined}
\input{Tables/openqa}


This section presents evaluation results on ANCE effectiveness and efficiency, and analyses on the Asynchronous learning. More evaluations and case studies can be found in Appendix.

\subsection{Effectiveness of ANCE Dense Retrieval}

The overall ranking accuracy in TREC Deep Learning Track benchmarks is presented in Table~\ref{tab:overall}. The main evaluation of DR methods is on their Retrieval accuracy from the ANN index; we also include their accuracy when Reranks top 100 documents retrieved by BM25.
% We separate the retrieval baselines from the reranking one for better comparisons. 
% For all DR methods, we mainly focus on their accuracy in the dense retrieval setting, using dot product in the ANN index, while we also include their results when used as a reranker on top of BM25 first stage retrieval.

ANCE empowers the DR model significantly outperforms all sparse retrieval baselines in all evaluation metrics. 
Not only it lead to 20\%+ NDCG gains over BM25 in all retrieval evaluations both passage retrieval and document retrieval, it also significantly outperforms the well-tuned best TREC traditional retrieval and best feature-based reranking models by large margins. Different from recent concerns on whether a single dense vector is sufficient for document DR, both ANCE (FirstP) and ANCE (MaxP) significantly advance the stage-of-the-art in document retrieval, without using any sparse information during retrieval---compared to DeepCT, which uses BERT to optimize sparse retrieval~\cite{dai2019transformer}, ANCE trained DR models enjoy 10\% better NDCG without replying on any BOW information. Similar advantages are also reflected in the MARCO Passage Retrieval in both MRR and recall.




Among all the learning mechanisms recently developed to train DR models, the best mechanism besides ANCE is to use a combination of BM25 negatives and random negatives: the sparse retrieval leads to a natural ``dictionary'' to select negatives for langauge related tasks, as discussed in multiple parallel work~\cite{gao2020complementing, ma2020zero, luan2020sparsedense, karpukhin2020dense, he2019momentum}. Yet there is almost always a 10\% gap from other methods to ANCE training---though all these approaches use the exact same DR model, the vanilla BERT-Siamese network. To the best of our knowledge, ANCE is the only method that enables dense retrieval to robustly outperform the best tuned sparse method in document ranking tasks. Section~\ref{sec:efficiency} further studies how the better negatives in the asynchronous learning of ANCE lead to this overwhelming effectiveness.

We found it promising to see BERT-Siamese, with ANCE training, nearly matches or even outperforms the interaction-based BERT reranker. This contradicts previous observations in Neu-IR, that the matches between query terms and document terms in the discrete BOW space is a necessity for neural ranking models~\cite{xiong2017knrm, guo2016deep, qiao2019understanding}. Many of the previous negative results upon BERT dual-encoders in Neu-IR perhaps are due to the challenges in model training rather than the network architecture. The same representation based BERT even outperforms the interaction-based BERT in document ranking. Not only that, in document retrieval, the bottleneck preventing end-to-end learned systems in many language AI systems, the ANCE trained DR model is less than 3\% away from the complex and state-of-the-art cascade IR pipeline which employs spare retrieval and then BERT Reranker, while only using the perhaps simplest dot product function in retrieval. 
In Section~\ref{sec:efficiency}, we discuss how this leads to very promising ``return of investiments'' (ROI) in computing resources.

\input{Tables/efficiency}
\subsection{Efficiency of ANCE Retrieval and Learning}
\label{sec:efficiency}

Table~\ref{tab.efficiency} measures the efficiency of different operations used in sparse retrieval, cascade IR pipeline, ANN dense retrieval, and ANCE's Asynchronous learning process.
Note that these numbers are measured in our commodity CPU/GPU server, with the open source toolkits we used. They may vary with different hardware, different implementation, paralleling, and distillation---though we expect the trend will remain mostly unchanged.

With batching, dot prod with FAISS ANN on CPU is sufficiently efficient. In high throughput environment such as commercial search, with sufficient query traffic to batch, fetching the document in the ANN index with dot prod is as efficient as from BM25's inverted index. 
Compared to Cascade IR, DR with BERT-Siamese enjoys much greater efficiency, especially online. The document encoding is calculated offline, i.e. in the crawling phrase of web search, and stored in the index; only the query encoding is required online, which requires less than 3ms and can be easily cached. In comparison, ranking with interaction-based BERT requires conducting inference on all the top K retrieved documents from BM25, which in theory is at least $O(K \times \frac{|q|+|d|}{|q|})$ times more expensive than DR ($|q|$ and $|d|$ refers to their lengths). In our experiment it requires more than one second per query, in comparison to DR's 11ms in high throughput environment, where efficiency matters the most. 

The cost Cascade IR with BERT ranker is often prohibitive latency wise or computing resource wise in many real systems, thus requires various approaches to speed up, e.g., to compute part of the transformer representations offline and cache them~\cite{}, to only use a few lower transformer layers~\cite{}, or to do task-specific distillation~\cite{}, all enforce certain efficiency-effectiveness trade-off. In comparison, our DR is 100 times more efficient, with 97\% accuracy, solely using a simple dot prod operation in the first stage retrieval.
This leads to remarkable ROI with reduced computing resource, energy consumption, and overhead on maintaining complicated pipelines.

In the ANCE Training phrase, Table~\ref{tab.efficiency} shows that the main bottleneck is not in the ANN part. Building the ANN Index or constructing the negative for the entire training query only takes seconds or minutes, which is perfectly fine in synchronous setting. However, the main bottleneck is to update the encodings of the document in the index, which requires a BERT inference of all the 8 Million training documents. This makes some type of asynchronous training almost inevitable in stochastic learning: the representation model is being updated per training batch, e.g., $n$ documents, $n<128$ per GPU. To keep the representations used in negative construction synchronous, one needs to refresh the encoding of all potential negatives, e.g. $m$ document, $m>1,000,000$, which is a $\frac{m}{n}\approx 1k$ times overhead just to avoid asynchronous training. Section~\ref{sec:Analyses} shows that asynchronous learning is effective enough and it is unnecessary to refresh the entire corpus's representation after each training batch.




\subsection{Analyses on ANCE Asynchronous Learning}
\label{sec:Analyses}
\input{Figures/fluct}

In this experiment we first analyze the main advantage of ANCE: stronger and more realistic negatives during training. Then we study the influence of delayed updates in the Asynchronous learning.



Figure~\ref{fig.neg overlap} shows the overlap of negatives used in training versus the negatives seen in actual dense retrieval in the testing stage, measured through the learning process on the same set sampled queries. 
% For each of these approaches, in each of \cx{TODO: XXX} training step, we 
Similar to the illustration in Figure~\ref{fig.motivation}, which is from the actual learned representations in ANCE(FirstP) on query ``what is the most popular food in Switzerland'', there is very low overlap between the training negatives, sampled from BM25 or Randomly, and the negatives seen in testing by their corresponding trained models. Only 11\% testing negatives appears in the BM25 negative pool and there is no overlap with the randomly sampled ones in training. The mismatch between training distribution and testing distribution risks optimizing DR models to undesired direction and perhaps was the main roadblock preventing DR to outperform sparse retrieval.

ANCE fundamentally eliminates this discrepancy by using the exact same approach in retrieval training instances and in testing. In the beginning of its training, as it is warmed up by BM25 Neg, ANCE already constructs negative instances with 60\% overlap. As the model converging, the ANCE negatives become closer to the testing negatives and eventually the two become the same, by definition. This is the sole difference between ANCE trained DR models with those DR baselines and itself alone elevates DR models outperform sparse retrieval in document ranking.

Figure~\ref{fig:fluct} illustrates the behavior of ANCE Asynchronous learning with different ANN index refreshing frequencies. When the refreshing rate is too low, the representation space used to construct training negatives is delayed too much from the up-to-date one being optimized. This leads to very fluctuating training curves and may even cause the model to diverge, e.g., in Figure~\ref{fig:fluct}.a, as the training distribution is too far away from optimal (though still better than not using ANCE negatives). As expected, refreshing the ANN index more frequently leads to much more smooth training curve, as shown in Figure~\ref{fig:fluct}.c., with the price of slower training speed. 
However, as shown in Figure~\ref{fig:fluct}.d, which is our choice, a 1:1 allocation of inferencer GPU and trainer GPU amounts is adequate to train the DR models effectively. More ablation studies of those hyper-parameter choices are included in Appendix.

In Appendix, we also include results in other retrieval tasks and examples of winning/losing queries of DR versus BM25. The t-SNE plots of all TREC DL evaluation queries, the same with Figure~\ref{fig.motivation}, and our intuitions on them are also included in Appendix.


==> Arxiv/evaluation.tex <==
\section{Evaluation Results}
\input{Tables/doc_pass_combined}

\begin{figure}\hspace*{-3cm}\CenterFloatBoxes
   \begin{floatrow}
       \ffigbox[\FBwidth]{\raisebox{-1\height}{\includegraphics[width=0.65\columnwidth]{Figures/overlap_line.pdf}}}{\caption{Training Neg Overlap vs Final KNN}\label{Dinah}}
        \ttabbox{\resizebox{0.45\textwidth}{!}{\input{Tables/efficiency_inference_tbl}}
         }{\caption{Efficiency of ANCE Inference and Training}\label{mytable}}
   \end{floatrow}
\end{figure}


\begin{figure}[htbp]
  \centering
  \hspace*{-1.5cm}\includesvg[width=1.2\columnwidth]{Figures/fluctuation.svg}
  \caption{ANCE learning fluctuation study}
\end{figure}



\subsection{Text Retrieval Effectiveness}

\cx{Results showing our performance gain over previous baselines in TREC Doc and passage ranking
\begin{enumerate}
    \item BM25
    \item Best BM25 + query expansion
    \item feature-based LeToR
    \item DeepCT
    \item BERT-Siamese (Zhuyun's paper)
    % \item reranking results of Roberta on ANCE and BM25 \lx{you mean retrieval? or reranking?}
\end{enumerate}
Also show inference time of these work.
}


\lx{checked with Chenyan, we will need that for document first} \cx{Yes and then paragraph.}




\cx{Results compare our training methods with other negative sampling. 
\begin{enumerate}
    \item Random negative
    \item in batch NCE
    \item BM25 negative
    \item BM25 warm up + in batch NCE
    \item BM25 + IB (FAIR paper)
    \item [TODO] BM25 warm up + Momentum NCE
\end{enumerate}
}
%  \ja{Should we show a comparison where we pick hard negatives just in one iteration Vs picking in multiple steps for convergence; most training exercises pick negatives once and here we say that picking it for every N step and then converging N steps is superior}
% }


\subsection{Dense Retrieval and ANCE learning Efficiency}
\cx{
o	A table measure the efficiency of the following on the document retrieval task, in our final setting:
	Time for sparse retrieval (BM25) per query (100 doc)
	Time of BERT Reranking (rerank top 100 of BM25)
	Time of dense retrieval (100 doc)
	The time cost in refreshing the ANN index in ANCE training, breaking down to:
•	ANN refreshing, including:
o	Time to infer the representation of the corpus
o	Time to build the ANN index
•	Batch training:
o	Time to fetch the top K (k=the number we used in the final model) negatives from ANN for each training batch
o	The time cost per training batch
}




\subsection{ANCE Learning Analyses}
\label{sec:ancenegatives}

% \begin{figure}
%     \centering
%     \input{Figures/fluctuation.svg}
% \end{figure}






% \input{Tables/efficiency_training_tbl}

\cx{Figures to show the negative overlaps of BM25 Neg, Rand Neg, ANCE neg, Versus ANN inference time negatives along the training curve of ANCE and BM25+Rand Neg}

\cx{Zoom in the ANCE learning process and demonstrate why ANCE is crucial and what is its effect in the learning process.
\begin{enumerate}
    \item Show the paired training loss curve and testing performance along the curve
    \item track and show the overlap of the ANCE negatives and BM25 negatives along the curve. Show the overlap and testing NDCG in these data points a) the overlap in the beginning of ANN refresh; b) in the middle between ANN refresh.
    \item also compare the negative overlap with in batch negatives (that there is very little overlap)
    \item compare the negative overlap at the end of each ANN refresh, show that the model learns stronger and stronger negatives. Also show the positive recall in top K of ANN at those data points \lx{I think end of each refresh basically means using query-inference from the beginning of next start checkpoint, but using doc inference from the previous checkpoint} \cx{query inference from the beginning of next start checkpoint is almost the same at the end of past checkpoint as they are only one backprop away?}
    \item \ao{is there any difference in learning speed, i.e. does ANCE help get the model to perform better faster or does it to allow training longer or both? \cx{Compared to which baseline? On doc, in batch negative or random all hurt, and just can't learn much, ANCE I think quickly passes them and far ahead. We can compare with BM25+IB (FAIR paper) on passage I think. TODO Lee: what is their learn curve look like? \ao{I was thinking to compare with BM25+IB}}}
\end{enumerate}}

\subsection{Case Studies}
\begin{figure}[tb]
  \centering
  \hspace*{-0.5cm}\includegraphics[width=1.2\columnwidth]{Figures/case_studies.pdf}
  \caption{Winning & Losing Case\lx{moving to native latex table below Table 4} }
\end{figure}

\input{Tables/case_study_tbl}

\cx{Show the wining cases and losing cases of ANN retrieval VS BM25. 
\begin{enumerate}
    \item  Plot the per query win/loss VS BM25 (the same style as in TREC DL Overview paper Figure 2 (this might leave in appendix)
    \item show winning case and losing examples of each
    \item \ao{what is our hole rate? are the holes good/bad, should we study this a bit? \cx{I think we can show it but as we are better than baseline I think we don't need to spend much time to study the hole rate, showing that we are better even with holes is good enough? \ao{sure, I'm just interested what the hole rate is and if it's large there might be something interesting}}}
\end{enumerate}
}






==> Arxiv/intro_v1.tex <==
\section{Introduction}



Many language systems rely on text retrieval to find relevant information  for later stages. For example,
search ranking~\cite{nogueira2019passage}, open domain question answering~\cite{chen2017reading}, and fact verification~\cite{yang2018hotpotqa, thorne2018fact} all first use text retrieval to find relevant information as the input to their later stage ranking, QA, and reasoning models.
All these later stage models enjoy the effectiveness from deep learning techniques~\cite{rajpurkar2016squad, wang2018glue}, while, in contrast, the first stage retrieval is still largely exact matching discrete bag-of-words~\cite{chen2017reading, zhaotransxh2020, yang2018hotpotqa, nogueira2019passage}.
Such sparse retrieval, e.g., BM25~\cite{bm25}, has various intrinsic challenges, i.e., vocabulary mismatch~\cite{croft2010search}, and leads to noises or missed information challenging or even impossible to recover in later stages~\cite{craswell2020overview, luan2020sparsedense, yang2018hotpotqa}


% The noisy and incomplete information brought in by the sparse first retrieval, limits the full potential of modern language AI systems, as t
% which brings in and missed information
% BM25~\cite{bm25}, unsupervised sparse retrieval using hand-crafted rules, is still a strong baseline and sometimes even the state-of-the-art, 40 years after its invention~\cite{zamani2018neural, karpukhin2020dense, luan2020sparsedense, lee2019latent}.
% The limited capability of the sparse first retrieval enforces a potential upper bound of modern language AI systems.
% The intrinsic challenge of sparse retrieval, i.e. vocabulary mismatch and language varieties~\cite{croft2010search}, brings in noisy and missed information in the first stage, which is challenging, sometimes impossible 
% for the later deep neural models to recover~\cite{yang2018hotpotqa, craswell2020overview}. 




% \cx{The importance of dense retrieval:
% \begin{enumerate}
%     \item resolve the bottleneck in e2e information system
%     \item unleash the full potential of neural methods in many downstream applications
%     \item unified and easier to maintain infrastructure
%     \item Also Pretrained LM and ANN inference are getting ready
% \end{enumerate}
% }
% \cx{The observations and challenges in recent progress:
% \begin{enumerate}
%     \item good for short passage but not as good on longer passage
%     \item reranking is promising but not yet fully e2e retrieval, many times have to combine with sparse model
%     \item even some permissive analyses that the capacity of encoding has to be very high for documents
% \end{enumerate}
% }

Dense retrieval (DR), which retrieves texts using learned distributed representations, is a promising potential direction to overcome this sparse retrieval bottleneck~\cite{lee2019latent, chang2020pre, luan2020sparsedense, gao2020complementing, ma2020zero, dhingra2020differentiable, karpukhin2020dense}: The representation space is fully learnable and can leverage the strength of pretraining, while the retrieval operation is sufficiently efficient thanks to the recent progress in Approximate Nearest Neighbor (ANN) search~\cite{johnson2019billion}.
One would expect dense retrieval to revolutionize the first stage retrieval, as deep learning has done in almost all language tasks, which, However, is not yet the case: Recent studies often found that dense retrieval with even pretrained language models under performs with BM25, especially on long texts~\cite{luan2020sparsedense, lee2019latent}, and DR is often used in combination and as an add-on to BM25~\cite{gao2020complementing, ma2020zero}.
The underwhelming performance even raises concerns whether it is reasonable to encoding the entire document into one dense vector~\cite{luan2020sparsedense}.
% , and the effectiveness of dense retrieval is mainly when combined with spare retrieval~\cite{gao2020complementing, ma2020zero}---as an add-on to BM25, but not yet a next-gen retrieval.

\input{Figures/motivation}



% \cx{Our solution:
% \begin{enumerate}
%     \item We identified the main bottleneck is actually in the training phrase, the mismatch between negatives seem in training and ANN inference
%     \item Developed a new training mechanism in the NCE framework, but instead of in-batch sampling, we directly do that in ANN, which is exact how the dense retrieval model is to be used
% \end{enumerate}
% }

In this paper we identify the main reason of such underwhelming performance of dense retrieval, especially on longer texts, is the learning part. Specifically, the mismatches of negatives sampled for training and the actually negatives in retrieval. 
% \ja{Previous sentence and next sentence are both technically strong and convey vital aspect of understanding; consider : Too many commas, suggest breaking down the long sentence for better readability}
In training, the negatives is either randomly sampled, selected in nearby batches, or from the sparse retrieval, following standard learning to rank settings~\cite{liu2009learning}. However, when testing, the trained model needs to retrieve the relevant documents in the entire corpus, e.g., via ANN, which is drastically different  from the negatives in sparse retrieval nor the random sampled negatives can provide the minutiae required for ranking among the top retrievals ($\mathsection$~\ref{sec:Analyses}). 


% \cx{More details of ANCE:
% \begin{enumerate}
%     \item We build ANN index with the doc representations
%     \item directly pick negatives from the ANN for each q and d+ label
%     \item refresh ANN after certain steps, as asynchronous updates
%     \item until converges in validation
% \end{enumerate}
% }

We eliminate this mismatch with Approximate nearest neighbor Noise Contrastive Estimation (ANCE), which follows the principle of NCE~\cite{gutmann2010noise, mnih2013learning, oord2018representation}, and selects stronger, \textit{more realistic}, negatives from an ANN index in learning. The ANN index includes the encodings of the documents/passages, from the same representation model being learned for the dense retrieval, and is parallelly updated and asynchronously refreshed as the optimization goes on. The negatives are sampled from this ANN index using the same retrieval function (dot product, e.g.), the same representation model (though delayed due to the asynchronous index update). 
This provides much stronger and more realistic negative instances---exactly the same as the retrieval model will face in inference time---and eliminate the discrepancy in the representation learning and testing.





% \cx{Our contribution as shown in experiments:
% \begin{enumerate}
%     \item The first to outperform all sparse retrieval, BM25 and beyond, as well as feature-based LeToR on TREC DL Doc task, a realistic, large scale, document retrieval task from Bing queries and documents.  
%     \item stronger than other training mechanisms: NCE, in batch, BM25+NCE, etc. (hopefully also momentum).
%     \item All with vanilla BERT-Siamese,  works for both doc ranking and passage ranking, with simple max-pooling or longformer on doc side.
% \end{enumerate}
% }

In TREC Deep Learning Track's large scale document and passage ranking benchmarks~\cite{craswell2020overview}, ANCE significantly boost the retrieval accuracy of dense retrieval. With ANCE training, the vanilla BERT-Siamese dual encoder, the same architecture used in several parallel research~\cite{luan2020sparsedense, gao2020complementing, ma2020zero}, significantly outperforms all dense retrieval baselines, many with same architecture but different training scheme, sparse retrieval methods, including BM25 and many upgraded variations, and even the two-stage retrieval and reranking state-of-the-art IR pipeline which uses BERT as the neural ranker.  
We found the later very impressive: the dot-product retrieval in the ANCE learned representation space provides more effective, more efficiency, and simpler solution than the existing state-of-the-art two-stage IR pipeline.
% the ANCE-learned model is a simple dot-product operation in the learned representation space, 
% it not only improves the effectiveness, but also simplifies and speeds up the system's pipeline.

This overwhelming performance is the first we have observed in dense retrieval.
In our studies we show how the negatives from sparse retrieval or other sampling method differ from the negatives dense retrieval models face in testing, and how ANCE fundamentally resolves this difference.
% the actual dense retrieval 
% and our analyses provide further insights and illustrate how ANCE effectively optimizes the representation for simpler and more accurate dense retrieval.
We also show how the ANN index refreshing influences the ANCE training and the necessity of fast asynchronous refreshing to keep the representations in the index on-pace with the representation being optimized. We plan to make our implementation of ANCE training and the asynchronous refreshing of ANN index publicly available to facilitate future research in representation learning. 




% \cx{Our insights:
% \begin{enumerate}
%     \item the main gain is from our ANCE training, without it, there is a clear gap in reranking and retrieval, and our analyses show how the gap of different negatives are resolved during the ANCE training.
%     \item More details in how/when to refresh index, the LR scheduling, warm up, and negative sampling, to shine lights of representation learning in other related tasks
%     \item case studies to show the different behavior of dense retrieval and sparse retrieval 
% \end{enumerate}
% }

==> Arxiv/openqair.tex <==
% \begin{table}[t]
%     \centering
%     \small
    \begin{tabular}{l|cccc|cccc} \hline \hline
         &   \multicolumn{4}{c|}{\textbf{Single Task Training}} 
         & \multicolumn{4}{c}{\textbf{Multi Task Training}}  \\ \hline
         & \multicolumn{2}{c}{\textbf{Natural Questions}} 
         & \multicolumn{2}{c|}{\textbf{TriviaQA}} 
         & \multicolumn{2}{c}{\textbf{Natural Questions}} 
         & \multicolumn{2}{c}{\textbf{TriviaQA}}  \\ \hline
         \textbf{Retriever} 
        &  {Top-20} & {Top-100}
        &  {Top-20} & {Top-100}
        &  {Top-20} & {Top-100}
        &  {Top-20} & {Top-100} \\ \hline
        BM25 & 59.1 & 73.7 & 66.9 & 76.7 & -- & -- & -- & -- 
        \\ 
        DPR & 78.4 & 85.4 & 79.4& 85.0 & 79.4 & 86.0 & 78.8 & 84.7 
        \\
        BM25 + DPR & 76.6 & 83.8 & 79.8 & 84.5 &  78.0 & 83.9 & 79.9 & 84.4
        \\ \hline
        ANCE & \textbf{81.9} & \textbf{87.5} & \textbf{80.3} & \textbf{85.3} & \textbf{82.1} & \textbf{87.9} & \textbf{80.3} & \textbf{85.2} \\
        \hline 
    \end{tabular}
% \end{table}

==> Arxiv/p_res.tex <==
\lx{this is placeholder template until numbers are fully replaced}
\begin{table*}[ht]
    \centering
    \small

        \begin{tabular}{l|cc|cc|cc} \hline \hline
    & \multicolumn{2}{c|}{\textbf{MARCO Dev}} 
    & \multicolumn{2}{c|}{\textbf{TREC Rerank}} 
    & \multicolumn{2}{c}{\textbf{TREC Retrieval}}
    \\ \hline  
           \textbf{Method}     
    &  \textbf{MRR@10} &  \textbf{Recall@1k}
     &  \textbf{NDCG@10} &  \textbf{Hole@10}
     &  \textbf{NDCG@10} &  \textbf{Hole@10}
    \\ \hline
    
{BM25}
& 0.20 &  ~ & ~ & ~ & ~ 
\\\hline
DeepCT~\cite{dai2019context} & Copy marco number and leave passage ones as n.a.\\ 
{TREC Best Retrieval}  & \\
{TREC Best Trad} &  \\
{Bert Ranker}  
& -- & -- & ~ & -- & -- & -- 
\\ \hline
{\textbf{Sentence-Bert}} & ~ & ~ & ~ & ~ & ~ & ~  \\
{w/ BM25 negative} 
& 0.299 & 0.928 & ~ & ~ & ~ & ~ 
\\ % /mnt/semi/kwtang/msmarco/20200505_2337_bm25_nll_first_ln_717533c8-74e0-4bbc-8747-d69d341c62f0/checkpoint-60000/

{w/ NCE} 
& 0.256 & 0.943 & ~ & ~ & ~ & ~
\\ % /mnt/semi/kwtang/msmarco/20200505_2337_bm25_nll_first_ln_717533c8-74e0-4bbc-8747-d69d341c62f0/checkpoint-60000/

{w/ IB} 
& 0.261 & 0.949 & ~ & ~ & ~ 
\\ % /mnt/semi/kwtang/msmarco/20200505_2337_bm25_nll_first_ln_717533c8-74e0-4bbc-8747-d69d341c62f0/checkpoint-60000/

{w/ BM25 + IB} 
& 0.311 & 0.952 & ~ & ~ & ~ & ~  \\ % mnt/semi/kwtang/msmarco/20200506_1937_nll_first_ln_9579aec6-2b94-400a-99d9-70b287a8e86c/checkpoint-90000/
\hline
{\textbf{Warmup from BM25}} & ~ & ~ & ~ & ~ & ~ & ~  \\

{w/ NCE} 
& 0.279 & 0.942 & ~ & ~ & ~ & ~ 
\\ % /mnt/semi/kwtang/msmarco/20200505_2337_bm25_nll_first_ln_717533c8-74e0-4bbc-8747-d69d341c62f0/checkpoint-60000/

{w/ IB} 
& 0.280 & 0.948 & ~ & ~ & ~ & ~ 
\\ % /mnt/semi/kwtang/msmarco/20200505_2337_bm25_nll_first_ln_717533c8-74e0-4bbc-8747-d69d341c62f0/checkpoint-60000/

%{w/ IB + BM25} 
%& ~ & ~ & ~ & ~ & ~ & ~ 
%\\ % /mnt/semi/kwtang/msmarco/20200505_2337_bm25_nll_first_ln_717533c8-74e0-4bbc-8747-d69d341c62f0/checkpoint-60000/

{w/ ANCE} & \textbf{0.330} & \textbf{0.959} & ~ & ~ & ~ & ~  \\ %../../../../glue_data/MSMarcoANN/rdot_clf_nll_4gpu_768d_t200_highlr_continue_with_2x_refresh/checkpoint-65000

\hline \hline
    \end{tabular}
     \caption{TREC DL Track 2019 Passage 
    \label{tab:passage_overal}}
\end{table*}



==> Arxiv/related.tex <==
\section{Related Work}

% \cx{NeurIR starts with representation based model: CDSSM~\cite{huang2013learning}, but later interaction-based are strong with cross attention~\cite{guo2016deep}, especially with relevance specific representations~\cite{xiong2017knrm}. BERT performs well in interaction model~\cite{nogueira2019passage} but the study how dense retrieval with BERT is just started.
% }

% \cx{Related work in dense retrieval: 
% Dense retrieval in OpenQA~\cite{lee2019latent}.
% Mix-batch NCE and BM25~\cite{karpukhin2020dense}.
% ReQA~\cite{ahmad2019reqa} and pretraining study of dense retrieval~\cite{chang2020pre}.
% The use of ANN dense retrieval in QA and pretraining: REALM~\cite{guu2020realm} and Reasoning~\cite{dhingra2020differentiable}.
% Recent parallel work that have to combine dense and sparse: empirical study~\cite{ma2020zero}, learn with sparse~\cite{gao2020complementing}, theory analyses and combination~\cite{luan2020sparsedense}.
% }

In neural information retrieval (Neu-IR), neural ranking models are categorized into representation-based and interaction-based, depending on whether they represent query and document separately, or model the detailed interactions between term pairs~\cite{guo2016deep}.
For example, BERT ranker~\cite{nogueira2019passage} takes the concatenated query-document sequence and models the term interactions with self-attention, thus is interaction-based, while BERT-Siamese is representation-based. 
Previous research found interaction-based models more effective then representation-based, that modeling the interaction between discrete query-document term pairs seemed a necessity~\cite{xiong2017knrm, dai2019deeper, qiao2019understanding}. \ao{sentence}


However, the advantage of interaction-based Neu-IR is only directly applicable in the reranking stage, as for each query, the model needs to know the to-be-scored candidate documents, which require a first-stage sparse retrieval to provide. To break this sparse retrieval bottleneck, researchers revisited the representation-based model with BERT for dense retrieval, leading to a series of progresses including the BERT dual-encoder latent retrieval in OpenQA~\cite{lee2019latent}, the ReQA OpenQA dense retrieval benchmark~\cite{ahmad2019reqa}, and customized pretraining for it~\cite{chang2020pre}, etc.
Nevertheless, especially in long document retrieval, the effectiveness of dense retrieval alone was underwhelming, that it has to be combined with, and serves as an ``add-on'' to, sparse retrieval~\cite{luan2020sparsedense, gao2020complementing, ma2020zero}; \ao{sentence} it was unclear whether it is possible to encode the entire document into one dense vector without losing too much information~\cite{luan2020sparsedense}.


Using Noise Constructive Estimation~\cite{gutmann2010noise, mnih2013learning} to construct stronger negative training instances are mostly recently by the contrastive representation learning framework in computer vision, for example, InfoNCE~\cite{oord2018representation}, SimCLR~\cite{chen2020simple}, and MoCo~\cite{he2019momentum, chen2020improved}. \ao{sentence} 
% More recently, in visual representation learning, MoCo improves InfoNCE and  constructs the negatives from a maintained queue of previous batches, using momentum updates to keep the representations in the queue up-to-date~\cite{he2019momentum, chen2020improved}. 
The technical choices in visual representation learning is different with in language, as language contains a natural ``dictionary''~\cite{he2019momentum}: NCE upon sampled random negatives is not as effective in learning language representations~\cite{karpukhin2020dense}. \ao{sentence}
Technical-wise, refreshing the ANN index in parallel has been recently utilized in REALM, where it is used to fetch contexts as input to the grounded language model, instead of as contrastive learning instances~\cite{guu2020realm}.
% ANCE can be viewed as natural next step of InfoNCE and MoCo with more global negatives from the ANN index of the entire corpus. This is supported by the asynchronous ANN refreshing with the representation learning, which has been recently utilized by REALM,
% though they use ANN to fetch contexts as input to the grounded language model, instead of as contrastive learning instances~\cite{guu2020realm}.




% With ANCE we demonstrate that 1) BERT-Siamese, the representation-based Neu-IR model, matches the effectiveness in the reranking setting with the BERT ranker, the interaction-based model, without requiring any term level interaction in the sparse representations; 2) dense retrieval, in the ANCE learned representation space, outperform the state-of-the-art sparse retrieval by itself, and nearly matches the accuracy of the cascade pipeline, while being much simpler and efficient.  



% Recently, similar ideas have been visited extensively in representation learning, for example, InfoNCE uses NCE to pick images that to contrast the representation of the image~\cite{oord2018representation}, and is a core component in the SimCLR framework for contrastive visual representation learning~\cite{chen2020simple}. MoCo improves InfoNCE and constructs the negatives by maintaining a queue of previous batches and their representations, which use momentum updates to keep a smooth encoding~\cite{he2019momentum, chen2020improved}. 








==> Impact.tex <==
\section*{Broader Impact}
% Authors are required to include a statement of the broader impact of their work, including its ethical aspects and future societal consequences. 
% Authors should discuss both positive and negative outcomes, if any. For instance, authors should discuss a) 
% who may benefit from this research, b) who may be put at disadvantage from this research, c) what are the consequences of failure of the system, and d) whether the task/method leverages
% biases in the data. If authors believe this is not applicable to them, authors can simply state this.

% Use unnumbered first level headings for this section, which should go at the end of the paper. {\bf Note that this section does not count towards the eight pages of content that are allowed.}


 For the past decades, in academic community we have been joking that every year we made 10\% progress upon BM25, but it had always been 10\% upon the same BM25; the techniques developed require more and more IR domain knowledge that might be unfamiliar to researchers in other related fields. For example, in OpenQA, document retrieval was often done with vanilla BM25 instead of the well-tuned BM25F, query expansion, or SDM.
In industry, many places build their search solutions upon open source solutions, such as Lucene and ElasticSearch, where BM25, a technique invented in the 1970s and 1980s, was incorporated as late as 2015~\cite{elasticbm25}; the required expertise, complex infrastructure, and computing resource make many missing out the benefits of Neu-IR.


With their effectiveness, efficiency, and simplicity, ANCE and dense retrieval have the potential to redefine the next stage of information systems and provide broader impacts in many fronts.
% the following fronts.

\textbf{Empower User with Better Information Access:} The effectiveness of DR is particularly prominent for exploratory or knowledge acquisition information needs. 
Formulating good queries that have term overlap with the target documents often requires certain domain knowledge, which is a barrier for users trying to learn new information.
A medical expert trying to learn how to build a small search functionality on her patient's medical records may not be aware of the terminology ``BM25'' and ``Dense Retrieval''.
By matching user's information need and the target information in a learned representation space, ANCE has the potential to overcome this language barrier and empower users to achieve more in their daily interactions with search engines.


\textbf{Reduce Computing Cost and Energy Consumption in Neural Search Stack:}
The nature of dense retrieval makes it straightforward to conduct most of the costly operations offline and reuse the pre-computed document vectors.
This leads to 100x better efficiency and will significantly reduce the hardware cost and energy consumption needed when serving deep pretrained models online. We consider this a solid step towards carbon neutrality in the search stack.


\textbf{Democratize the Benefit of Neural Techniques:} Building, maintaining, and serving a cascade IR pipeline with the advanced pretrained models is daunting and may not lead to good ROI for many companies not in the web search business. In comparison, the simple dot product operation in a mostly pre-computed representation space is much more accessible. Faiss and many other libraries provide easy-to-access solution of efficient ANN retrieval; our (to be) released pretrained encoders and ANCE open-source solution will fill in the effectiveness part. Together we will democratize the recent revolutions in neural information retrieval to a much broader audience and end-users.

 



==> Tables/efficiency.tex <==

\begin{figure}\TopFloatBoxes


   \begin{floatrow}
    \ttabbox{\resizebox{0.5\textwidth}{!}
         {\input{Tables/efficiency_inference_tbl}}}
         {\caption{Efficiency of Offline and Online (per query and 100 documents) operations. 
         }
         \label{tab.efficiency}}
    \hspace{0.2cm}   
    
    \ttabbox{\resizebox{0.4\textwidth}{!}
     {\input{Tables/prod}}}
      {\caption{Offline gains in the first stage retrieval of a commercial search engine at different Corpus size, encoding Dimension, and dense Retrieval setting. 
    %   The gains are measured by adding ANCE to the same DR model.
    %   using the same training labels.
    %   , same training data, same pretraining starting point, with ANCE versus without ANCE.
      }
      \label{tab.prod}
      }
   
   \end{floatrow}
\end{figure}



==> Tables/floatefficiency.tex <==
% \vspace{-1cm}\newlength{\oldintextsep}
\setlength{\oldintextsep}{\intextsep}
\setlength\intextsep{-1pt}
\begin{wraptable}{tr}{0.48\textwidth}
\resizebox{\textwidth}{!}{\input{Tables/efficiency_inference_tbl}
\caption{Efficiency of Sparse and Dense IR.\label{tab.efficiency}\vspace{-0.2cm}}
}
\end{wraptable}         

==> Tables/floatprod.tex <==

\begin{wraptable}{r}{0.4\textwidth}
\small
\resizebox{\textwidth}{!}{\caption{Offline gains in the first stage retrieval of a commercial search engine at different Corpus size, encoding Dimension, and dense Retrieval setting. 
      \label{tab:prod}
  } \input{Tables/prod}}
\end{wraptable}

==> Tables/openqa_retrieval_full.tex <==
\begin{table}[t]
    \centering
    % \small
     \caption{Answer Coverage at Top-K on 
         Natural Questions (NQ) and Trivial QA (TQA) in the setting from ~\citet{karpukhin2020dense}. Top-5/10 baseline results are produced using their open-source code.    \label{tab:openqa} \vspace{-0.5mm}  
     } 
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|cccc|cccc} \hline \hline
         &   \multicolumn{4}{c|}{\textbf{Single Task}} 
         & \multicolumn{4}{c}{\textbf{Multi Task}}  \\ \hline
         
         & \multicolumn{2}{c}{\textbf{Natural Questions}} 
         & \multicolumn{2}{c|}{\textbf{Trivia QA}} 
         & \multicolumn{2}{c}{\textbf{Natural Questions}} 
         & \multicolumn{2}{c}{\textbf{Trivia QA}}  \\ \hline
         \textbf{Retriever} 
            &  {Top-5/10} 
        &  {Top-20/100}
        &  {Top-5/10}
        &  {Top-20/100} 
        &  {Top-5/10} 
        &  {Top-20/100}
        &  {Top-5/10}
        &  {Top-20/100} \\ \hline
        BM25 & 
        & 59.1/73.7 
        &
        & 66.9/76.7 
        &
        & --/-- 
        &
        & --/-- 
        \\ 
        DPR &  68.3/74.9
        & 78.4/85.4 
        & 70.9/75.7
        & 79.4/85.0 
        &
        & 79.4/86.0 
        &
        & 78.8/84.7 
        \\
        BM25+DPR & 
        & 76.6/83.8 
        &
        & 79.8/84.5 
        &
        &  78.0/83.9 
        &
        & 79.9/84.4
        \\ \hline
        ANCE &  \textbf{71.8}/\textbf{77.8}
        & \textbf{81.9}/\textbf{87.5} 
        & \textbf{72.3}/\textbf{76.5}
        & \textbf{80.3}/\textbf{85.3} 
        &
        & \textbf{82.1}/\textbf{87.9} 
        &
        & \textbf{80.3}/\textbf{85.2} \\
        \hline 
    \end{tabular}
    }
\end{table}

==> Tables/openqa_topvals.tex <==
% \begin{table}[t]
%     \centering
%     \small
    \begin{tabular}{l|cccc} \hline \hline
         \multicolumn{1}{c}{Retriever}
         & \multicolumn{1}{c}{Top-5}
         & \multicolumn{1}{c}{Top-10}
         & \multicolumn{1}{c}{Top-20}
         & \multicolumn{1}{c}{Top-100} \\ \hline
        
        \textbf{NQ} & & & &
        \\
        DPR & 68.3 & 74.9 & 80.0 & 86.0
        \\ 
        ANCE & 71.8 & 77.8 & 81.9 & 87.5 
        \\ \hline
        \textbf{TQA} & & & &
        \\
        DPR & 70.9 & 75.7 & 79.4 & 85.0
        \\
        ANCE & 72.3 & 76.5 & 80.3 & 85.3
        \\ \hline 
    \end{tabular}
% \end{table}
